Large-System Analysis of Massive MIMO with Optimal M-MMSE Processing

We consider the uplink of a Massive MIMO network with $L$ cells, each comprising a BS with $M$ antennas and $K$ single-antenna user equipments. Recently, [1] studied the asymptotic spectral efficiency of such networks with optimal multicell minimum mean-squared error (M-MMSE) processing when $M\to \infty$ and $K$ is kept fixed. Remarkably, [1] proved that, for practical channels with spatial correlation, the spectral efficiency grows unboundedly, even with pilot contamination. In this paper, we extend the analysis from [1] to the alternative regime in which $M,K\to \infty$ with a given ratio. Tools from random matrix theory are used to compute low-complexity approximations which are proved to be asymptotically tight, but accurate for realistic system dimensions, as shown by simulations.

==> appendices.tex <==
\newpage
\begin{figure*}
 \begin{align}
 {\bf T}_{j}^{\star} &= \left(\left(\frac{1}{M}\left(\frac{\frac{MK}{P} \nu}{1+\mu^\star} + \frac{\frac{MK}{P}\nu\alpha(L-1)}{1+\alpha\mu^\star}\right)+\frac{1}{M}\frac{MK}{P} (1-\nu)\overline L\right){\bf A}{\bf A}^{\Htran} + \frac{1}{M{\rho}}{\bf I}_M\right)^{-1}\\&=\left(\frac{K}{P}\underbrace{\left(\frac{\nu}{1+\mu^\star} + \frac{\nu\alpha(L-1)}{1+\alpha\mu^\star}+ (1-\nu)\overline L\right)}_{\eta^\star\overline L}{\bf A}{\bf A}^{\Htran}+ \frac{1}{M{\rho}}{\bf I}_M\right)^{-1}
  \end{align}
  \hrule
  \begin{align}\label{boundT}
\frac{M}{KL}\frac{1}{\underbrace{\max_{jli}||\vect{\Phi}_{jlli}||_2 + \max_{jli}||\vect{R}_{jli} - \vect{\Phi}_{jlli}||_2 + \frac{1}{KL}}_{\varsigma}}{\bf I}_M \preceq {\bf T}_j^{\star} \preceq \frac{M}{KL}\frac{1}{\underbrace{\min_{jli} \lambda_{\min}(\vect{R}_{jli} - \vect{\Phi}_{jlli})}_{\eta}}{\bf I}_M
\end{align}
\hrule
  \end{figure*}
\section*{Appendix B}
Under Assumption~\ref{assumption_3}, the matrix ${\bf T}_j^{\star}$ can be bounded as in \eqref{boundT} at top of the page. Hence, from \eqref{sigma_jk_1} we have that 
%\begin{align}\notag
%\big[\vect{B}_{jk} \big]_{j,j} = \frac{1}{M}\tr \left(  \vect{\Phi}_{jjjk} {\bf T}_{j}^{\star}\right) &\mathop\le^{{(a)}} ||\vect{\Phi}_{jjjk}||_2\frac{1}{M}\tr \left(  {\bf T}_{j}^{\star}\right)\\&\mathop\le^{{(b)}}\frac{M}{KL}\frac{||\vect{\Phi}_{jjjk}||_2}{\eta}
%\end{align}
%where $(a)$ follows from $\tr \left( \vect{A} \vect{B}\right) \le \| \vect{A} \|_2\tr \left( \vect{B}\right)$ and $(b)$ comes from the right-hand-side of \eqref{boundT}. Also, we have that 
%\begin{align}
%\big[\vect{B}_{jk} \big]_{j,j} = \frac{1}{M}\tr \left(  \vect{\Phi}_{jjjk} {\bf T}_{j}^{\star}\right) &\mathop\ge^{{(a)}} \frac{M}{KL} \frac{1}{\varsigma}\frac{1}{M}\tr \left(  \vect{\Phi}_{jjjk} \right)
%\end{align}
%where $(a)$ comes from the left-hand-side of \eqref{boundT}. Putting these results together yields
\begin{align}\label{B.3}
 &\!\!\!\!\!\!\frac{M}{KL} \frac{1}{\varsigma}\frac{1}{M}\tr \left(  \vect{\Phi}_{jllk} \right) \le \big[\vect{B}_{jk} \big]_{l,l}\le \frac{M}{KL}\frac{1}{\eta}\frac{1}{M}\tr \left(  \vect{\Phi}_{jllk} \right)
% \\
%  &\!\!\!\!\!\!\frac{M}{KL} \frac{1}{\varsigma}\frac{1}{M}\tr \left(  \vect{\Phi}_{jl'lk} \right) \le \big[\vect{B}_{jk} \big]_{l,l'}\le \frac{M}{KL}\frac{1}{\eta}\frac{1}{M}\tr \left( \vect{\Phi}_{jl'lk} \right)\label{B.3.1}
\end{align}
which implies that the first term in \eqref{eq:general result_1} is of order $\Omega(M/K)$. For the second term in \eqref{eq:general result_1}, we notice that
\begin{align}\label{B.4}
 \frac{1}{L-1} \tr \left(  \vect{B}_{jk}^{[jj]} \right) \vect{I}_{L-1}\preceq \vect{B}_{jk}^{[jj]} \preceq \tr \left(  \vect{B}_{jk}^{[jj]} \right) \vect{I}_{L-1}.
\end{align}
By using ${\bf x}^{\Htran}\vect{A}{\bf x}^{\Htran} \le {\bf x}^{\Htran}\vect{C}{\bf x}^{\Htran}$ if $\vect{C}-\vect{A} \succeq \vect{0} $, we have that
\begin{align}\notag
{\big(\vect{b}_{jk}^{[j]}\big)}^{\Htran}&\left(  {\bf I}_{L-1}+ \vect{B}_{jk}^{[jj]}\right)^{-1}\!\!\!\vect{b}_{jk}^{[j]} \mathop\ge^{{(a)}} \frac{\sum\limits_{l=1}^{L-1}{(\big[\vect{B}_{jk}^{[jj]}\big]_{ll}})^2}{1 + \tr \left(  \vect{B}_{jk}^{[jj]} \right) } \\&\mathop\ge^{{(b)}}\frac{(\frac{M}{KL})^2 \frac{1}{\varsigma^2} \sum\limits_{l=1,l\ne j}^{L} \big(\frac{1}{M}\tr \left(  \vect{\Phi}_{jllk} \right)\big)^2}{1 + \frac{M}{KL} \frac{1}{\eta} \sum\limits_{l=1,l\ne j}^{L} \frac{1}{M}\tr\left(  \vect{\Phi}_{jllk} \right)}
\end{align}
where $(a)$ and $(b)$ follow from the right-hand-sides of \eqref{B.4} and \eqref{B.3}, respectively. Similarly, we have that 
\begin{align}\notag
{\big(\vect{b}_{jk}^{[j]}\big)}^{\Htran}&\left(  {\bf I}_{L-1}+ \vect{B}_{jk}^{[jj]}\right)^{-1}\!\!\!\vect{b}_{jk}^{[j]} \mathop\le^{{(a)}} \frac{\sum\limits_{l=1}^{L-1}{(\big[\vect{B}_{jk}^{[jj]}\big]_{ll}})^2}{1 +  \frac{1}{L-1}\tr \left(  \vect{B}_{jk}^{[jj]} \right) } \\&\mathop\le^{{(b)}}\frac{(\frac{M}{KL})^2 \frac{1}{\varsigma^2} \sum\limits_{l=1,l\ne j}^{L} \big(\frac{1}{M}\tr \left(  \vect{\Phi}_{jllk} \right)\big)^2}{1 + \frac{M}{KL}  \frac{1}{L-1}\frac{1}{\eta} \sum\limits_{l=1,l\ne j}^{L} \frac{1}{M}\tr\left(  \vect{\Phi}_{jllk} \right)}.
\end{align}
%Therefore, it can be lower bounded as follows:
%\begin{align}\notag
%{\big(\vect{b}_{jk}^{[j]}\big)}^{\Htran}&\left(  {\bf I}_{L-1}+ \vect{B}_{jk}^{[jj]}\right)^{-1}\!\!\!\vect{b}_{jk}^{[j]} \\\notag&\mathop\ge^{{(a)}} \frac{\sum\limits_{l=1}^{L-1}{(\big[\vect{B}_{jk}^{[jj]}\big]_{ll}})^2}{1 + \|\vect{B}_{jk}^{[jj]} \|_2} \\&\mathop\ge^{{(b)}}\frac{\sum\limits_{l=1}^{L-1}{(\big[\vect{B}_{jk}^{[jj]}\big]_{ll}})^2}{1 + \frac{M}{KL} \frac{1}{\eta} \sum\limits_{l=1,l\ne j}^{L} \frac{1}{M}\tr\left(  \vect{\Phi}_{jllk} \right)}\\&\mathop\ge^{{(c)}}\frac{(\frac{M}{KL})^2 \frac{1}{\varsigma^2} \sum\limits_{l=1,l\ne j}^{L} \big(\frac{1}{M}\tr \left(  \vect{\Phi}_{jllk} \right)\big)^2}{1 + \frac{M}{KL} \frac{1}{\eta} \sum\limits_{l=1,l\ne j}^{L} \frac{1}{M}\tr\left(  \vect{\Phi}_{jllk} \right)}
%\end{align}
%where $(a)$ follows from $\tr \left( (\vect{I}+\vect{A})^{-1} \vect{B}\right) \ge \frac{1}{1+\| \vect{A} \|_2}\tr \left( \vect{B}\right)$, $(b)$ from the right-hand-side of \eqref{B.4} and \eqref{B.3}, and $(c)$ from the left-hand-side of \eqref{B.3}.







\section*{Appendix C}
If the channel is modelled as in \eqref{corr_model}, then $\vect{Z}_{j} $ and $\vect{\Theta}_{jll'i}$ are diagonal matrices with entries
%\begin{align}\label{cov_model}
%\vect{\Phi}_{jlli} &= \diag\left({\phi}_{jli}(1),\ldots,{\phi}_{jli}(M)\right)\\
%\vect{Z}_{j} &= \diag\left({z}_{j}(1),\ldots,{z}_{j}(M)\right)
%\end{align}
%with 
%\begin{align}
%{\phi}_{jli}(m) = \frac{\big({r}_{jli}(m)\big)^{2}}{\sum\limits_{n=1}^{L} {r}_{jni}(m) + \frac{1}{\rho^{\rm{tr}}}}
%\end{align}
\begin{align}\label{zjm}
{z}_{j}(m) = \sum\limits_{l=1}^{L} \sum\limits_{i=1}^{K} ({r}_{jli}(m) - {\phi}_{jli}(m)) + \frac{1}{{\rho}}
\end{align}
and
      \begin{align}
{\Theta}_{jll'i}(m) = \frac{{r}_{jli}(m){r}_{jl'i}(m)}{\sum\limits_{n=1}^{L} {r}_{jni}(m) + \frac{1}{\rho^{\rm{tr}}}} = {\phi}_{jli}(m)\frac{{r}_{jl'i}(m)}{{r}_{jli}(m)}.
  \end{align}
Therefore, we have that 
    \begin{align}
\mu_{jlk} = \frac{1}{M} \sum\limits_{m=1}^{M}\frac{{\phi}_{jlk}(m)}{\frac{1}{M}\sum\limits_{l'=1}^{L}\sum\limits_{i=1}^{K}\frac{{\phi}_{jl'i}(m) }{1 + \mu_{jl'i}} + \frac{1}{M}{z}_j(m)}.
  \end{align}
  Solving with respect to $\{\mu_{jlk}\}$ yields
      \begin{align}
\mu_{jlk}^\star =  \frac{1}{M}\sum\limits_{m=1}^{M} \frac{{\phi}_{jlk}(m)}{\varsigma_{j}^\star(m)}
  \end{align}
  with $\varsigma_{j}^\star(m)$ given by \eqref{varsigma_j} (where we have used \eqref{zjm}). If two cells are active, we have that
\begin{align}\label{SNR_two_cell}
\overline{\gamma}_{1k}^{\rm {ul}} = \big[\vect{Z}_{1k} \big]_{1,1} - \frac{\big[\vect{Z}_{1k} \big]_{1,2}\big[\vect{Z}_{1k} \big]_{2,1}}{1+ \big[\vect{Z}_{1k} \big]_{2,2}}
\end{align}
with $\big[\vect{Z}_{1k} \big]_{l,l'}=\frac{1}{M}\sum\limits_{m=1}^{M} \frac{{\phi}_{1lk}(m)}{\varsigma_1^\star(m)} \frac{{\beta}_{1l'k}(m)}{{\beta}_{1lk}(m)}$. Putting all the results together yields \eqref{gamma_diagonal}.
  
  \section*{Appendix D}
Following \cite[Sec.~IV]{Hoydis2013}, we assume that
   \begin{align}\label{sigma_jk}
{\bf H}_{jj} = {\bf A}{\bf V}_{jj} \quad {\bf H}_{jl} = \sqrt{\alpha}{\bf A}{\bf V}_{jl}
  \end{align}
  where ${\bf A}\in\mathbb{C}^{M\times M}$ is an arbitrary unitary matrix $M\times M$ matrix, ${\bf V}_{jj}\in\mathbb{C}^{M\times K}$ are standard
complex Gaussian matrices and $\alpha \in (0,1]$ is an intercell
interference factor. This implies that
 \begin{align}
\vect{\Phi}_{jlli} = \begin{cases}
 \nu{\bf I}_M & {\textrm{if }} j=l  \\ \\ 
\alpha \nu {\bf I}_M & {\textrm{if }} j\ne l
\end{cases}
\end{align}
with $\nu = \frac{{\rho^{\rm{tr}}}}{1+{\rho^{\rm{tr}}}\overline L}$ with $\overline L = 1 + \alpha(L-1)$. Also, we have that
   \begin{align}
\vect{Z}_{j}  = \Big(\frac{K}{M} (1-\nu)\overline L + \frac{1}{M\rho}\Big){\bf I}_M.
\end{align}
By using the above results, we obtain
 \begin{align}
 {\bf T}_{j}^{\star} =\left(\frac{K}{M}\overline L\eta^\star {\bf I}_M + \frac{1}{M{\rho}}{\bf I}_M\right)^{-1}
  \end{align}
  where
   \begin{align}
 \eta^\star =  \frac{1}{\overline L}\left(\frac{\nu}{1+\mu^\star} + \frac{\nu\alpha(L-1)}{1+\alpha\mu^\star}\right)+ (1-\nu)
   \end{align}
   with $\mu^\star$ being the solution of the set of fixed point equations. The latter can be computed with standard calculus, but it is not required for the subsequent analysis.
By using the above results, we have that 
 \begin{align}  \notag
 &  \big[\vect{Z}_{1k} \big]_{1,1} = \frac{1}{M}\tr \left(  \vect{\Phi}_{11k} {\bf T}_{1}^{\star}\right) \\\notag&=\frac{\nu}{M}\tr \left(  \left(\frac{K}{M}\overline L\eta^\star {\bf I}_M + \frac{1}{M{\rho}}{\bf I}_M\right)^{-1}\right)\\\notag&=\nu\left(\frac{K}{M}\overline L\eta^\star + \frac{1}{M{\rho}}\right)^{-1}\\&=\frac{\nu M}{{K\overline L\eta^\star}+\frac{1}{{\rho}}}\triangleq X.
   \end{align}
Assume for simplicity that $L=2$. By using similar steps as for $\big[\vect{Z}_{1k} \big]_{1,1}$, we obtain 
   \begin{align}
{\bf I}_2+ \vect{Z}_{1k}  = 
  \left[ {\begin{array}{cc}
   1+X & \alpha X \\
   \alpha X & 1+\alpha^2 X \\
  \end{array} } \right]
   \end{align}
such that \eqref{SNR_two_cell} reduces to
%    \begin{align}\label{sigma_jk}
%\big[\vect{Z}_{jk} \big]_{l,l'}= \begin{cases}
%\nu\frac{M}{K}\eta^\star& {\textrm{if }} l=l'  \\ \\ 
%\alpha^2\nu\frac{M}{K}\eta^\star & {\textrm{if }} l\ne l'
%\end{cases}
%\end{align}
\begin{align}\notag
\overline{\gamma}_{1k}^{\rm {ul}} &=X - \frac{(\alpha X)^2}{1+\alpha^2 X}=\frac{1}{X^{-1}+\alpha^2} \\
&= \frac{1}{\underbrace{\frac{1}{M{\rho}\nu}}_{\text{Noise}}+\underbrace{\frac{K}{M}\frac{\overline L}{\nu}\eta^\star}_{\text{Non-coherent Interference}}+\underbrace{\alpha(\overline L-1)}_{\text{Coherent interference}}}.
\end{align}
The above result is in a similar form of  \cite[Eq. (30)]{Hoydis2013}.
